Near Instance-Optimality in Differential Privacy

We develop two notions of instance optimality in differential privacy, inspired by classical statistical theory: one by defining a local minimax risk and the other by considering unbiased mechanisms and analogizing the Cramer-Rao bound, and we show that the local modulus of continuity of the estimand of interest completely determines these quantities. We also develop a complementary collection mechanisms, which we term the inverse sensitivity mechanisms, which are instance optimal (or nearly instance optimal) for a large class of estimands. Moreover, these mechanisms uniformly outperform the smooth sensitivity framework on each instance for several function classes of interest, including real-valued continuous functions. We carefully present two instantiations of the mechanisms for median and robust regression estimation with corresponding experiments.

==> discussion.tex <==
\section{Discussion}

\jcdcomment{ Say something about how while we do unbiased stuff for
  optimality, it would be much cooler to do some asymptotics. This would
  move us from 1930s Cram\'{e}r-Rao to 1970s local asymptotics in
  statistics.  }

